LLaVA-Plus: Learning to Use Tools for Creating Multimodal Agents

LLaVA-Plus is a general-purpose multimodal assistant that expands the capabilities of large multimodal models. It maintains a skill repository of pre-trained vision and vision-language models and can activate relevant tools based on users' inputs to fulfill real-world tasks. LLaVA-Plus is trained on multimodal instruction-following data to acquire the ability to use tools, covering visual understanding, generation, external knowledge retrieval, and compositions. Empirical results show that LLaVA-Plus outperforms LLaVA in existing capabilities and exhibits new ones. It is distinct in that the image query is directly grounded and actively engaged throughout the entire human-AI interaction sessions, significantly improving tool use performance and enabling new scenarios.

==> images_tex/llava_plus_pipeline.tex <==
\begin{figure}[h!]
\centering  
\vspace{-4mm}
\includegraphics[width=\textwidth]{resources/llava_plus_pipeline2.pdf}
\vspace{-1mm}
\caption{\shortname{} pipeline.}
\label{fig:llava_arch}  
  \vspace{-3mm}
\end{figure}

==> tables_tex/ablation_thoughts.tex <==
\begin{table}[t!]
    \centering
    \begin{subtable}{1.0\textwidth} 
    \centering 
     \scalebox{0.8}{
    \begin{tabular}{l|cccc|cccc}
    \toprule
    &  \multicolumn{4}{c}{\textbf{LLaVA-Bench (COCO)}} & \multicolumn{4}{c}{\textbf{LLaVA-Bench (In-the-Wild)}} \\
         &  
        {\footnotesize Conv.} & {\footnotesize Detail} & {\footnotesize Reasoning} & {\footnotesize All}
        & {\footnotesize Conv.} & {\footnotesize Detail} & {\footnotesize Reasoning} & {\footnotesize All}\\ \midrule
        LLaVA   & 82.0  & 69.1  & 92.6  & 81.2  & 42.6  &	51.9  &	68.9 & 57.1  \\ 
        LLaVA (Tools in Test)  & 56.2  & 67.9  & 53.3  & 59.1 & 40.7  &	48.1  &	51.2 & 47.5   \\ 
       %  \midrule
        \rowcolor{Gray} 
        \shortname{} (All Tools)   & 81.6  & 74.5  & 95.7  & \textbf{83.9}  & 65.5 &	56.8 &	79.1 &	\textbf{69.5}  \\ 
         \rowcolor{Gray} 
        \shortname{} (Fly)   & 76.2  & 72.2  & 92.3  & 80.4 & 45.2 & 	50.4 &	72.6 &	59.1  \\ 
        \rowcolor{Gray} 
        \shortname{} (Fly) (no \texttt{thoughts})   & 76.6  & 70.4  & 90.7  & 79.4 & 38.8 & 	39.8 &	59.8 &	48.7  \\ 
        \midrule
        GPT4Tools & 75.3 &	53.8 &	86.9 & 	72.1  & 31.1 & 27.1 & 54.1 & 40.7\\
    \bottomrule
    \end{tabular}
    }
    \vspace{-2mm} 
     \vspace{1mm}
      \end{subtable} 
    \caption{Ablation of the impacts of \texttt{thoughts}.}
    \label{tab:ablation_thoughts}
\end{table}



==> tables_tex/comparison_data_model_variants.tex <==
\begin{table}
  \begin{minipage}{0.99\textwidth}
\centering  
\vspace{-4mm}
\scalebox{0.65}{
\begin{tabular}{l p{5.5cm} p{6.5cm} p{6.5cm} }
\toprule
 \multicolumn{4}{l}{\bf Comparisons of training data for variance models.}  \\
\midrule
 & \multicolumn{3}{l}{\includegraphics[height=4.5cm]{resources/girl_cart.jpg}}  \\
 & \multicolumn{3}{l}{{\tiny Source: COCO training data. Id: 569536 }}\\
Model & LLaVA & LLaVA-Plus (A) &  LLaVA-Plus (B) \\
\addlinespace
User & \multicolumn{2}{l}{Can you segment the girl and the cart in the image and describe their relationship?} & Can you segment the girl and the cart in the image and describe their relationship? \\
\addlinespace
AI & \multirow{3}{5.5cm}{The girl in the image is a young child, and she is sitting in a shopping cart. The cart is being pulled by the child, and it appears that she is holding onto the handles of the cart. The relationship between the girl and the cart is that the girl is using the cart to transport herself, possibly to move around a store or a public area. The cart is designed to be pulled by a child, making it a convenient and safe mode of transportation for the young girl.}  & \textbf{``thoughts"} To accurately segment and identify the girl and the cart in the image, we can leverage the grounding\_dino model for open-set detection and the segmentation model SAM. Integrating these models will enable us to generate a comprehensive summary of the segmented subjects. & \multirow{3}{6.5cm}{Sure! I segment and identify the little girl and the cart in the image. \\
\qu- Centered in the image, a little girl is discernible with bounding box coordinates [0.35, 0.37, 0.66, 0.97]. She's seen actively maneuvering a cart within the airport's ambiance. \\
\quad - To the bottom left of the image, a cart can be pinpointed, bounded by the coordinates [0.0, 0.57, 0.69, 1.0]. It's laden with various luggage items, indicating travel preparations or arrivals. \\
\quad The interaction between the girl and the cart epitomizes a typical airport scenario: a traveler utilizing the cart to facilitate her movement with luggage. This tableau, whether signifying an arrival or departure, encapsulates the vibrancy and expectation inherent to air travel.\\} \\
& &\textbf{``actions"} [{"API\_name": "grounding\_dino+sam", "API\_params": {"caption": "little girl and cart ."}}] \\
& & \textbf{``value"} I will use grounding\_dino+sam to help to answer the question. Please wait for a moment. \\
\addlinespace
Tool& & \textit{Run tools: Grounding DINO + SAM} \\
\addlinespace
User & & grounding\_dino+sam model outputs:  {'boxes': [[0.35, 0.37, 0.66, 0.97], [0.0, 0.57, 0.69, 1.0]], 'logits': [0.58, 0.41], 'phrases': ['little girl', 'cart']} \\
& & Can you segment the girl and the cart in the image and describe their relationship? \\
\addlinespace
AI & & \textbf{``thoughts"} Thanks to the output of grounding\_dino+sam. I can answer the question better. \\
& & \textbf{``actions"} [] \\
& & \textbf{``value"} Sure! I segment and identify the little girl and the cart in the image. \\
& & \quad - Centered in the image, a little girl is discernible with bounding box coordinates [0.35, 0.37, 0.66, 0.97]. She's seen actively maneuvering a cart within the airport's ambiance. \\
& & \quad - To the bottom left of the image, a cart can be pinpointed, bounded by the coordinates [0.0, 0.57, 0.69, 1.0]. It's laden with various luggage items, indicating travel preparations or arrivals. \\
& & \quad The interaction between the girl and the cart epitomizes a typical airport scenario: a traveler utilizing the cart to facilitate her movement with luggage. This tableau, whether signifying an arrival or departure, encapsulates the vibrancy and expectation inherent to air travel.\\
\bottomrule
\end{tabular}
}
\vspace{2mm}
\captionof{table}{Example \shortname{} for object detection.}  
\label{tab:data_comp_different_model}  
  \end{minipage}
\end{table}

==> tables_tex/model_variants.tex <==
\begin{table}[!ht]
    \centering
    \scalebox{0.7}{
    \begin{tabular}{l|lll}
    \toprule
        \textbf{Model} & \textbf{Training Data} & \textbf{Using Tools} & \textbf{Training Cost}\\ 
        \midrule
        LLaVA-7b & Baseline model & No tools &  \\ 
        \midrule
        LLaVA-Plus-7b (A1) & LLaVA Instruction Data (150k)~\cite{liu2023visual} & Trigger tools\\
        LLaVA-Plus-7b (A2) & LLaVA Instruction Data (150k)~\cite{liu2023visual} + LLaVA Tools Instruction Data (81k) & Trigger tools\\
        LLaVA-Plus-7b (B) & LLaVA Instruction Data (150k)~\cite{liu2023visual} + LLaVA Tools Instruction Data (81k) & All Tools \\
    \bottomrule
    \end{tabular}}
    \caption{Model variants of LLaVA-Plus.}
    \label{table:model_variants}
\end{table}
